Video Referring Expression Comprehension via Transformer with Content-conditioned Query

Video Referring Expression Comprehension (REC) aims to localize a target object in videos based on the queried natural language. Recent improvements in video REC have been made using Transformer-based methods with learnable queries. However, we contend that this naive query design is not ideal given the open-world nature of video REC brought by text supervision. With numerous potential semantic categories, relying on only a few slow-updated queries is insufficient to characterize them. Our solution to this problem is to create dynamic queries that are conditioned on both the input video and language to model the diverse objects referred to. Specifically, we place a fixed number of learnable bounding boxes throughout the frame and use corresponding region features to provide prior information. Also, we noticed that current query features overlook the importance of cross-modal alignment. To address this, we align specific phrases in the sentence with semantically relevant visual areas, annotating them in existing video datasets (VID-Sentence and VidSTG). By incorporating these two designs, our proposed model (called ConFormer) outperforms other models on widely benchmarked datasets. For example, in the testing split of VID-Sentence dataset, ConFormer achieves 8.75% absolute improvement on Accu.@0.6 compared to the previous state-of-the-art model.

==> section/intro-ref.tex <==
\section{Introduction} \label{sec:intro}
Referring Expression Comprehension (REC)~\cite{hu2017modeling,hu2016natural,yu2016modeling,yu2017joint} aims to locate the image region described by the natural language query. This task has attracted extensive attention from both academia and industry, due to its wide applications, such as visual question answering~\cite{antol2015vqa}, image/video analysis~\cite{anderson2018bottom}, and relationship modeling~\cite{hu2017modeling}. %During the past few years, most previous works address REC in images ~\cite{wang2019neighbourhood,yang2019cross,yu2018mattnet,liao2020real,yang2019fast,mao2016generation}. 
Recently, with the increasing number of videos online, grounding the target object in the video domain is becoming an emerging requirement. %Some recent attempts~\cite{zhou2018weakly,vasudevan2018object,chen2019weakly,zhang2020does,feng2021siamese} begin to conduct REC in the video domain. 
Different from image REC, video REC~\cite{zhou2018weakly,vasudevan2018object,chen2019weakly,zhang2020does,feng2021siamese} is more challenging since it needs to deal with both complex temporal and spatial information.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{ContFormer/figs/query_tube.pdf}
	\vspace{-0.8em}
	\caption{The distribution of queries generated by our Content aware mechanism(marked in \textcolor{red}{red}) and traditional mechanism(marked in \textcolor{blue}{blue} )  }
	\vspace{-0.5em}
	\label{fig:query_tube}
\end{figure}

Recently, with the development of transformer [], DETR-like methods~\cite{carion2020end} have been demonstrated effective in object detection areas, which get rid of the manually-designed rules, dataset-dependent hyper-parameters, and post-processing steps. Following this pipeline, the primary work TubeDETR~\cite{yang2022tubedetr} customizes DETR model for video REC. Specifically, it introduces a video-text encoder and a space-time decoder, where several learnable queries are set up. This plain method brings noticeable performance improvements with clear designs compared with previous ones. 
Note TubeDETR inherits the fundamental design of DETR that uses a fixed number of learnable queries to respond to a limited quantity of semantic entities in a closed set configuration. Clearly, REC does not hold this condition as the language descriptions in REC work in an open-ended environment. It is true that existing REC datasets have limited semantic space that only a number of entities frequently appear, so a constant number of queries in the DETR framework can work in most cases as a compromise. Regarding this, we believe exploiting a dynamic query generation mechanism to produce language- and video-related features can address this challenging referring relationship in the open-world setting.

% 这一段我按自己理解写的，可能和方法不对应，需要改一下。
%In this paper, we propose a xxx . It is a transformer-based model to leverage video and text features to make visual- and text-guided queries for spatiotemporal detection. With these queries, we further convert them into xxx conditioned on visual features with a transformer decoder. Then, we build a cascade head to predict time stamps first and then predict spatial bounding boxes. xxx

Moreover, current video REC annotations only consider the correspondence between sentences and the described objects. Empirically, we contend that the nouns (\ie, subject or object) in a sentence are important to carry the overall meaning, \eg, ``\texttt{cat}" and ``\texttt{fox}" in Figure~\ref{fig:align&accu}(a) already cover the objects of interest. Therefore, the detailed alignment and differentiation between the mentioned noun objects and the corresponding visual areas (\ie, object areas or patches, \eg, the red and green dotted boxes in Figure~\ref{fig:align&accu}(a)) provide fruitful localization clues.
This asks the model to implicitly attend to keywords for matching visuals. We suppose enabling a REC model to highlight partially crucial text descriptions can make video REC more tractable. 
%\emph{2) Lack of fine-grained alignments.}  This fine-grained correlation, however, is overlooked in current Transformer-based methods.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{ContFormer/figs/align&accu.pdf}
	\vspace{-0.5em}
	\caption{(a) \textbf{The motivation of fine-grained alignments.} The certain \emph{regions} (\ie, object areas) of the frame are usually more salient and highly overlapped with \emph{nouns} in the sentence containing semantic meanings. (b) \textbf{Comparisons of the convergence curves} between TubeDETR~\cite{yang2022tubedetr} and our ContFormer.}
	%\vspace{-3em}
	\label{fig:align&accu}
\end{figure}



        


%\emph{2) Lack of fine-grained alignments.} Empirically, we find that the noun (\ie, subject or object) in a sentence is important to carry the overall meaning. Accordingly, certain patches (\ie, object areas) of the frame are usually more salient and highly overlapped with the semantic meanings. For example in Figure~\ref{fig:align_example}, the sentence contains two instances, \ie, ``\emph{cat}" and ``\emph{fox}". The detailed alignment and differentiation between the mentioned query objects and the corresponding visual areas provide localization clues. This fine-grained correlation, however, is overlooked in current Transformer-based methods. 


% 这个地方方法可以再具体些，类似第18行的写法
Based on the above analysis, we propose a novel xxx in Trans\textbf{former} (dubbed as \textbf{ContFormer}). We contend that the content-independent query is better suitable to the open-ended grounding scenarios than that using a preset amount of ones.
%is the main cause of the slow convergence. 
To this end, we propose to generate query embeddings conditioned on the video contents. Specifically, we set up a fixed number of bounding boxes across the frame. Then the cropped and pooled regional features are transformed into the query features of the transformer decoder. Compared to the conventional high-dimension learnable queries, our region-based features introduce more salient prior. For example in Figure~\ref{fig:query_tube}, these two video clips with different natural language sentences are from a same video. Our content-aware query adaptive focuses on region-of-interest according to the input query sentence while the pure learnable one focuses on fixed region. Besides, we also notice a faster convergence process when introducing content information (\cf, Figure~\ref{fig:align&accu}(b)).



Besides, to provide fine-grained alignment between text and videos, we contribute a semi-automatic entity generation pipeline to argument existing video REC datasets with more fine-grained text annotations, and the matched alignment losses to leverage these new supervisions. In REC annotations, we collect VID-Entity and VidSTG-Entity datasets (\cf, Figure~\ref{fig:dataset_example}) with spaCy tools and manual check, which annotate \emph{region-phrase} labels by grounding specific phrases in sentences with the bounding boxes in the video frames. To further use these detailed annotations, we also propose a fine-grained alignment loss. We first compute the similarity scores between each query-word pair. Then, we adopt the Hungarian algorithm~\cite{kuhn1955hungarian} to select the query matching the target bounding box. Supervised by the annotations of VID-Entity and VidSTG-Entity datasets, the InfoNCE loss is applied to map the fine-grained matched pair to be close.

We make three contributions in this paper:
\begin{itemize}[topsep=0pt, partopsep=0pt, leftmargin=13pt, parsep=0pt, itemsep=3pt]
	\item We contend that the current query design leads to the slow convergence process in Transformer-based video REC methods. To this end, we propose to generate content-conditioned queries based on the frame context.
	%\item Beyond the coarse-grained region-sentence one, we build two datasets (\ie, VID--Entity and VidSTG--Entity) and a fine-grained alignment loss to enhance the fine-grained \emph{region-phrase} alignment.
	\item Beyond the coarse-grained region-sentence one, we augment the current datasets with additional annotations and propose a fine-grained alignment loss to enhance the fine-grained \emph{region-phrase} alignment.
	\item Experimental results show that our ContFormer achieves state-of-the-art performance on both trimmed and untrimmed video REC benchmarks. 
\end{itemize}

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.95\textwidth]{figs/ContFormer_pipline.pdf}
	\vspace{-0.5em}
	\caption{The schematic illustration of our ContFormer. The video and text modalities are extracted by the modality-specific backbones and fused through the Transformer encoder. A novel content-aware query generation module is proposed for the Transformer decoder to generate content-conditioned query features. The overall pipeline is optimized by the bi-partial matching loss and our proposed entity-aware contrastive loss.}
	\label{fig:ContFormer_pipeline}
	%\vspace{-2mm}
\end{figure*}

==> table_fig/K_R.tex <==
\begin{table}[t]
\vspace{-0.5em}
\caption{Comparison of performance with various $T$ and spatial resolution on the VID-Entity testing set. }
\vspace{-0.5em}
\renewcommand\arraystretch{1.1}
%\setlength{\tabcolsep}{5pt}
\label{table:KR}
\begin{center}
%\resizebox{\linewidth}{!}{
\begin{tabular}{ccc}
\toprule
\textbf{$T$} & \textbf{Resolution} & \textbf{Accu.@0.5} \\
\midrule
15  & 800 & 66.38  \\
20 & 672 &\textbf{67.17}\\
25 & 576 &65.93\\
35 & 480 &59.28\\
\bottomrule
\end{tabular}
%}
\end{center}
\end{table}

==> table_fig/M_R.tex <==
\begin{table}[t]
\vspace{-0.5em}
\caption{Comparison of performance with various maximum of $T$ and spatial resolution on the VidSTG-Entity testing set. }
\vspace{-0.5em}
\renewcommand\arraystretch{1.1}
%\setlength{\tabcolsep}{5pt}
\label{table:MR}
\begin{center}
%\resizebox{\linewidth}{!}{
\begin{tabular}{cccc}
\toprule
\textbf{$T$} & \textbf{Resolution} & \textbf{m\_tIoU} & \textbf{m\_vIoU} \\
\midrule
 100 & 288&42.16&27.31 \\
 150 & 256 &43.33&27.56\\
 200 & 224 &\textbf{44.21}&\textbf{28.08}\\
\bottomrule
\end{tabular}
%}
\end{center}
\end{table}

==> table_fig/accu_epoch.tex <==
\begin{figure}[t]
	\centering
	%\setlength{\abovecaptionskip}{0.0cm}
	%\setlength{\belowcaptionskip}{-0.2cm}
	\includegraphics[width=0.4\textwidth]{figs/accu_epoch.pdf}
	\vspace{-0.5em}
	\caption{Comparison of Accu.@0.5 between content-aware query (marked in \textcolor{red}{red}) and content-agnostic query (marked in \textcolor{blue}{blue}).}
	%\vspace{-3em}
	\label{fig:accu_epoch}
\end{figure}

==> table_fig/ecl_dataset.tex <==
\begin{table}[t]
\vspace{-0.5em}
\caption{Comparison of performance with or withou Entity-aware Contrastive Loss (ECL) }
\vspace{-0.5em}
\renewcommand\arraystretch{1.1}
%\setlength{\tabcolsep}{5pt}
\label{table:ecl_dataset}
\begin{center}
%\resizebox{\linewidth}{!}{
\begin{tabular}{ccc}
\toprule
\textbf{Method} & \textbf{ECL} & \textbf{Accu.@0.5} \\
\midrule
\multirow{2}{*}{Yang \emph{et al.} (\emph{w/}) LSTM }&\ding{55} & 54.78  \\
&\ding{51} & 56.13 \\
\cdashline{1-3}[2pt/2pt]
\multirow{2}{*}{Co-grounding} &\ding{55} & 60.25  \\
& \ding{51} &63.88\\
\cdashline{1-3}[2pt/2pt]
\multirow{2}{*}{ContFormer (Ours)} & \ding{55} &62.10\\
& \ding{51} &67.17\\
\bottomrule
\end{tabular}
%}
\end{center}
\end{table}

==> table_fig/vid_sota_figs.tex <==
\begin{figure*}[tb]
	\centering
	\begin{minipage}{0.49\textwidth}

        \vspace{-0.5em}
        \renewcommand\arraystretch{1.1}
        %\setlength{\tabcolsep}{2pt}
        \label{table:VID-entity}

        \begin{center}
        %\resizebox{\linewidth}{!}{
        %\begin{tabular}{cp{1cm} cp{0.3cm} cp{0.3cm} cp{0.3cm}}
        \begin{tabular}{ccccccccccccccc}
        %\begin{tabular}{lx{15}x{15}x{15}}
        \toprule
        %\textbf{Methods} & \textbf{Accu.@0.4} & \textbf{@0.5} & \textbf{@0.6} \\
        \multirow{2}*{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Accu.@}} \\
        \cmidrule{2-4}
        %& 0.4 & 0.5 & 0.6 & & (\%) \\
        & 0.4 & 0.5 & 0.6  \\
        \midrule
        Yang \emph{et al.} (\emph{w/} BERT) & - & 52.39 & -  \\
        Yang \emph{et al.} (\emph{w/} LSTM) & - & 54.78 & -  \\
        %\hdashline
        %\midrule
        DVSA+Avg & 36.2 & 29.7 & 23.5 \\
        DVSA+NetVLAD & 31.2 & 24.8 & 18.5  \\
        DVSA+LSTM & 38.2  & 31.2 & 23.5  \\
        GroundeR+Avg & 36.7 & 31.9 & 25.0 \\
        GroundeR+NetVLAD & 26.1 & 22.2 & 15.1  \\  
        GroundeR+LSTM & 36.8 & 31.2 & 27.1  \\
        \cdashline{1-4}[2pt/2pt]
        First-frame tracking & - & 36.97 & -  \\
        Middle-frame tracking & - & 44.00 & - \\
        Last-frame tracking & - & 36.26 & -  \\
        Random-frame tracking & - & 40.20 & -\\
        \cdashline{1-4}[2pt/2pt]
        WSSTG & 44.60 & 38.20 & 28.90 \\
        Co-grounding & 63.35  & 60.25 & 53.89  \\
        \cdashline{1-6}[2pt/2pt]
        \textbf{ContFormer (Ours)} & \textbf{70.40} & \textbf{67.27} & \textbf{62.64} \\
        \bottomrule
        \end{tabular}
		\caption{Comparison (\%) with state-of-the-art methods on VID-Entity dataset.}
%}
\end{center}
	\end{minipage}
%	\hspace{0.5in}
	\begin{minipage}[h]{0.49\textwidth}
		\centering
		\includegraphics[width=0.7\linewidth]{ContFormer/figs/accu_loss.pdf}
	\caption{(a) Comparison of Accu.@0.5 between content-aware query (marked in \textcolor{red}{red}) and content-agnostic query (marked in \textcolor{blue}{blue}). (b) Comparison of loss curve of content-aware query (marked in \textcolor{red}{red}) and content-agnostic query (marked in \textcolor{blue}{blue}).}
		\label{fig:layers}
	\end{minipage}%
\end{figure*}

